Redes sociales, participaci\'on ciudadana y la hip\'otesis del slacktivismo: lecciones del caso de "El Bronco" / Social Media, Civic Engagement, and the Slacktivism Hypothesis: Lessons from Mexico's "El Bronco"

El uso de las redes sociales tiene consecuencias positivas o negativas en la participaci\'on ciudadana? La gran parte de los intentos por responder a esta pregunta incluyen datos de la opini\'on p\'ublica de los Estados Unidos, por lo que nosotros ofrecemos un estudio sobre un caso significativo de M\'exico, donde un candidato independiente utiliz\'o las redes sociales para comunicarse con el p\'ublico y rehuy\'o de los medios de comunicaci\'on tradicionales. Dicho candidato, conocido como "El Bronco", gan\'o la carrera por la gubernatura del estado al derrotar a los candidatos de los partidos tradicionales. Adem\'as, gener\'o una participaci\'on ciudadana que se ha mantenido m\'as all\'a del d\'ia de las elecciones. En nuestra investigaci\'on analizamos m\'as de 750 mil mensajes, comentarios y respuestas durante m\'as de tres a\~nos de interacciones en la p\'agina p\'ublica de Facebook de "El Bronco". Examinamos y demostramos que las redes sociales pueden utilizarse para dar cabida a una gran cantidad de interacciones ciudadanas sobre la vida p\'ublica m\'as all\'a de un acontecimiento pol\'itico. Does social media use have a positive or negative impact on civic engagement? The "slacktivism hypothesis" holds that if citizens use social media for political conversation, those conversations will be fleeting and vapid. Most attempts to answer this question involve public opinion data from the United States, so we offer an examination of an important case from Mexico, where an independent candidate used social media to communicate with the public and eschewed traditional media outlets. He won the race for state governor, defeating candidates from traditional parties and triggering sustained public engagement beyond election day. In our investigation, we analyze over 750,000 posts, comments, and replies over three years of conversations on the Facebook page of "El Bronco".

==> margins.tex <==
% margins.tex

% import calc
\usepackage{calc}

%
\newlength{\myrightmargin}
\newlength{\myleftmargin}
\newlength{\mytopmargin}
\newlength{\mybottommargin}

% Change these settings to change the margins
\setlength{\myrightmargin}{1.0in}
\setlength{\myleftmargin}{1.0in}
\setlength{\mytopmargin}{0.75in}     
\setlength{\mybottommargin}{0.75in} 
\setlength{\oddsidemargin}{0.0in}   % extra room on inside side

%%% use margin settings to set width variables
\setlength{\evensidemargin}{0 in}
\setlength{\marginparsep}{0 in}
\setlength{\marginparwidth}{0 in}
\setlength{\hoffset}{\myleftmargin - 1.0in}
\setlength{\textwidth}
  {8.5in -\myleftmargin -\myrightmargin -\oddsidemargin}

%%% use margin settings to set height variables
\setlength{\voffset}{\mytopmargin -1.0in}
\setlength{\topmargin}{0 in}
\setlength{\headheight}{12 pt}
\setlength{\headsep}{20 pt}
\setlength{\footskip}{36 pt}
\setlength{\textheight}
  {11.0in-\mytopmargin-\mybottommargin-\headheight-\headsep-\footskip}

==> preamble.tex <==
% preamble.tex

% enclose any latex in \comment{} to suppress it
\newcommand{\comment}[1]{}
\newcommand{\citeNP}[1]{\cite{#1}}

\usepackage{graphicx}
\usepackage{multicol}
\usepackage{times}
\usepackage{floatflt}
\graphicspath{{./}{figures/}}

% NO psfig -- pdflatex does not support it ...
% \usepackage{psfig}
% \psfigurepath{./:figures/}
% \DeclareGraphicsRule{.eps.gz}{eps}{.eps.bb}{'gunzip -c #1}

\newcommand{\upline}{\vspace*{-\baselineskip}}
\newcommand{\up}{\vspace*{-6pt}}
\newcommand{\downline}{\vspace*{\baselineskip}}
\newcommand{\sep}{~~~~~~~~~~}

% this hardcodes the bib name, which we don't want to do.
% \renewcommand{\thebibliography}[1]{\section*{References Cited}
% \addcontentsline{toc}{section}{References Cited}\list
%  {[\arabic{enumi}]}{\settowidth\labelwidth{[#1]}\leftmargin\labelwidth
%  \advance\leftmargin\labelsep
%  \usecounter{enumi}}
%  \def\newblock{\hskip .11em plus .33em minus -.07em}
%  \sloppy\clubpenalty4000\widowpenalty4000
%  \sfcode`\.=1000\relax}

% fix this to specify width and height, and solve for the margins
\input{margins}

% \oddsidemargin 0.2cm
% \evensidemargin 0cm
% \textwidth 16.0cm
% \topmargin -1.25cm
% \textheight 22.94cm

% remove parindent, squeeze grafs
\setlength{\parindent}{0in}
\setlength{\parskip}{1ex}

\def\nibf#1{\noindent\textbf{#1}}


==> priornsf.tex <==
% priornsf.tex
\vspace{-1pc}
\subsection{Results from Prior NSF Support}
\label{sec:priornsf}
\vspace{-0pc}

\begin{wrapfigure}{l}{15pc}
\vspace{-2pc}
  \begin{center}
    \hspace{0pc}{\includegraphics[width=14.5pc]{pics/assets_captioning2}}
  \end{center}
\vspace{-.8pc}
  \caption{Scribe in action at a session at the ACM ASSETS 2014 conference. The photo shows Scribe's real-time captions displayed on a big screen for the audience, along with Scribe typists and their laptops. Five conference attendees recruited 15min prior to the session provided real-time captioning.}
\vspace{.2pc}
\label{fig:assets}
\end{wrapfigure}

Dr. Bigham is the PI of \textbf{HCC:Small:Collaborative Research IIS-1218056 and IIS-1218209}, ``Real-Time Captioning by Groups of Non-Experts for Deaf and Hard of Hearing Students'' (7/12 - 6/16);  \textit{Intellectual Merit:} The award resulted in Scribe, an end-to-end system in which a small group of  on-demand, non-expert typists, who individually cannot type at real-time speaking rates, collectively do real-time captioning with performance approaching a professional stenographer \cite{Lasecki2012UIST} (Best Paper nomination at ACM UIST 2012). Subsequent work showed slowing down audio for each worker decreased per-word latency from 4.3s to 3.3s \cite{Lasecki2013CHI}  (CHI 2013 Best Paper nomination). Partial captions are merged together using multiple sequence alignment via weighted-A* beam search with heuristics derived from captionist performance for real-time runtime \cite{Naim2013NAACL,scribequality}. Scribe affords new flexibility in how captions can be used by Deaf and Hard of Hearing (DHH) students to improve accessibility. Eye-tracking studies informed guidelines for usability and readability of real-time captions \cite{Kushalnagar2014tcASSETS,Kushalnagar2014TACCESS,Kushalnagar2014SIGACCESS,Lasecki2014W4A,Kushalnagar2013w4a,Kushalnagar2012assets}, culminating in a pause and highlighting interface that received the Best Paper award at W4A 2014 \cite{Lasecki2014W4A}. \textit{Broader Impacts:} 25 undergraduates, including 18 underrepresented DHH students, participated in all aspects of the research process.  Five students 
co-authored peer-reviewed papers ~\cite{Kushalnagar2014tcICCHP,Kushalnagar2014tcASSETS,Kushalnagar2014pASSETS}. A resulting multimedia player interface (AccessibleViews) isused by DHH students during programming tutorials at the Rochester Institute of Technology. Dr. Bigham explored commercializing Scribe in the NSF I-Corps Program (\#1338678) and via an SBIR Award (\#1448616).


\vspace{0.4pc}
Dr. Bigham was the PI of \textbf{HCC:Small: Collaborative Research \#IIS-1116051}, ``MobileAccessibility - Bridge to the World for Blind, Low-Vision, and
Deaf-Blind People'' (7/2011 - 6/2014); {\em Intellectual Merit}: VizWiz is a mobile application that lets blind users take a picture from their existing mobile phones, speak a question, and receive answers from people on the web quickly. Results include creating and evaluating abstractions that turn existing sources of crowd work into nearly real-time human computation \begin{wrapfigure}{r}{12pc}
\vspace{-1.4pc}
  \begin{center}
    \hspace{0pc}{\includegraphics[width=11pc]{pics/dytective}}
  \end{center}
\vspace{-.8pc}
  \caption{A screenshot of Dytective showing one of several exercises designed to test cognitive skills associated with dyslexia.}
\vspace{-1.2pc}
\label{fig:dytective}
\end{wrapfigure}  \cite{vizwiz,legion,chorus}, design considerations for human-backed access technology \cite{human-powered-at-design}, studies of what blind people want to know about \cite{visual-challenges}, and approaches for supporting blind photography \cite{zhong-scanning,blind-photography,easysnap}. {\em Broader Impact}: From 2011-2015, more than 8,000 users asked VizWiz nearly 100,000 questions, which were answered in less than a minute on average. \textbf{CAREER \#IIS-1149709}, ``Closed-Loop Crowd Support for People with Disabilities'' (1/2012 - 12/2016); {\em Intellectual Merit}: This work explored ways for multiple crowd workers to collectively assist people with disabilities (primarily blind people). Results include developing the general “Crowd Agent” model for abstracting multiple crowd workers as a single individual \cite{crowdagents} to assume control of an inaccessible interface \cite{legion}, have a conversation with the user about their visual surrounding \cite{view,chorus}, and code large amounts of video data quickly \cite{glance}. {\em Broader Impact}: PI Bigham created a new course on crowdsourcing\footnote{course materials are online at http://www.programthecrowd.com}, and led a programming course for blind high school students incorporating social computing and 3D printing \cite{youthslam2013}. A key component of the crowdsourcing course is to have students spend substantial time as crowd workers. Four graduate students (2 women) and ten undergraduate researchers (5 women) were supported.

\vspace{0.4pc}
Dr. Bigham is a PI of \textbf{HCC:Small \#IIS-1618784}, ``Early Dyslexia Detection and Support at Scale to Help Students Succeed in School'' (7/1/2016 - 6/30/2019); {\em Intellectual Merit}: Current approaches to dyslexia detection are quite expensive, time consuming, and require an expert; our Dytective game   detects dyslexia with more than 90\% accuracy after 15 minutes of playing a game \cite{dytective}. Our Dytective U software targets interventions mapped to specific cognitive skills for which each child has difficulty (Figure \ref{fig:dytective}),  {\em Broader Impact}: Dytective has been used by nearly 10,000 children and we are actively working with schools to deploy Dytective U. Dr. Luz Rello (Co-PI) recently received the 2016 International Dyslexia Association ``New Researcher Award," recognizing her work on dyslexia\footnote{https://dyslexiaida.org/2016-award-recipients}.

==> questions.tex <==
a) I remvoed the part of the algorithms to find adequete work. is this a good idea. I focused more on the skill development. 

==> title.tex <==
\newcommand{\projtitle}{Redes sociales, participaci\'on ciudadana y la hip\'otesis del \textit{slacktivismo}:  lecciones del caso de ``El Bronco''
}

%Supporting Career Growth and Retention of Rural Adults in Crowd Work Marketplaces


==> title2.tex <==

\newcommand{\projtitle}{Redes sociales, participaci\'on ciudadana y la hip\'otesis del \textit{slacktivismo}:  lecciones del caso de ``El Bronco''
}


==> trash.tex <==
crowd market tasks and/or with specific work practices. 



https://www.sharelatex.com/project/59cbf84565ef6f46c946dadd



%Researchers have recently explored mentoring programs between experienced workers and novices to tackle the problem of crowd worker/education \cite{}. However, these approaches usually relay on experts investing time in teaching others, which can delay them from their own work.


%The lack of guidance limits the type of things that workers can learn, and the type of career opportunities they have access to. 



This is generally


However, most crowdsourcing platforms have not gone after this opportunity. As a result, the majority of workers are left alone without a clear path on how to develop their skills.








Working with our local partner ACHIEVA, we will: {\em (i)} conduct in-lab and long-term studies to understand how adults with autism could benefit from crowd working platforms, the problems they face in using current platforms, and how new tools may be beneficial; {\em (ii)} create a machine learning task recommendation engine and a user-facing queueing tool to help workers find suitable work efficiently and reduce the unpaid time workers spend ``finding" work rather than doing work; {\em (iii)} develop ``skill ladders'' to help workers improve their current skills and develop new skills while they work; and {\em (iv)} create tools that allow crowd workers with autism to work together to find work, share work, and exchange tips on working better together.






Three objectives embody this proposal. First, with ``SkillLadders'' we will  enable professional skill development while doing volunteer work. Second, `MicroMentoring'' will allow volunteers to receive quality professional feedback from experts but, without burdening the experts. Third, ``ProfessionalStreamer'' will study effective ways for experts to streamline and share professional advice to volunteers without volunteers having to invest a great amount of time and resources in the activity. To accomplish these objectives, the PIs will follow a user-centered design process and execute longitudinal evaluations in the wild. 






https://www.sharelatex.com/project/59cbf84565ef6f46c946dadd







%\vf{Overall comments: \\ 1 . The motivation may be large, it takes quite a while to really read what you are proposing. I think you can shorten it by saying that online learning platforms have failed to prepare workforce development in rural areas because X, and Y. Then you say, we propose to use crowd markets as an alternative solution to get money while learning.\\ 2. Is there a theory or grounds that suggests that this approach will be successful? This should be discussed in the introduction though. If there is not, then at least mention a few studies showing that this direction can be promising. \\ 3. Given that is so focused on rural communities, I sense that some reviewers will say that this is not general. You may want to consider generalized this for any person, and then mention that you will be focusing on rural areas since this is a great tool for them and good for testing this approach.}

%while online education is accessible, they have problem X and Y.
%We will investigate an alternative solution to prepare workforce development which can be useful in particular in rural communities.
%This solution is based on crowd markets

%Mike Mikalajunas
%Development programs help foster workforces that grow professionally, and adapt to the changing needs of the economy, employers, and workers themselves. Having  strong workforce development programs is crucial as it is estimated that by 2040 most individuals  will be constantly changing their jobs throughout their professional careers. People, therefore, need mechanisms through which they can ensure that they will continuously have marketable skills and knowledge. Creating strong workforce development programs also becomes important when we consider that currently almost 40 percent of employers in the US cannot find people with the skills they want, even for entry-level jobs. 60 percent of employers complain that their work applicants lack the skills and knowledge they need. This ``skill gap'' means that a large number of individuals are never hired, producing a massive pool of untapped talent. This has critical consequences, including economic under-performance, social unrest, and individual despair.
%Professional development programs help foster workforces that grow professionally, and adapt to the changing needs of the economy, employers, and workers themselves. However, few workers have access to workforce development programs. There are several reasons for this shortage of programs. First, it is usually only specific businesses who can afford to provide development options to their workforces. The high cost of delivering such programs generally arises because workers need to invest time in taking the training, leading them to delay the completion of their regular labour or forcing them to invest time outside their normal working hours, which generates additional costs to both the company and themselves. Second, most organizations lack the knowledge of how to generate flexible development programs that adapt to the changing needs of workers. This lack of flexibility leads to outdated programs that impede workforce development. 







and retain volunteers to adquiere particular skills via video streams. 



%The goal of this proposal is to investigate the development of computational techniques that include a more diverse set of learners in online education. 




The main goal of this proposal is to investigate the development of computational techniques that include a more diverse set of learners in online education. 



retain learners as long as possible. In particular, this proposal investigates the development of learning platforms using crowd market systems that offer a payment while learning. 


\vf{The overall objective of this proposal is to investigate the development of platforms that retain learners as long as possible. In particular, this proposal investigates the development of learning platforms using crowd market systems that offer a payment while learning. } This proposal's research objective is to investigate interactive systems and computational techniques that enables professional development 


transform crowd markets into platforms that enable professional growth while completing paid crowd work.



The main research question of this proposal is: can we create platforms or systems that enable professional development while doing paid work?







Rural adults, for instance, believe that time spent learning online is time that they are not earning money. Online learning is not a feasible option for them, since their priority is to earn money to survive. 

a) integrating rural workers into crowd markets; and b) facilitating workers' professional growth directly on existing crowd markets. This extends the boundaries of crowdsourcing research, which has focused on empowering requesters. Research that does look at workers has studied more the design of new crowd markets, or helping workers to organize. To accomplish these objectives, this research will produce: 1) techniques and patterns to facilitate the participation of rural workers and enable professional growth in crowd markets; 2) scientific results that uncover the strengths and weaknesses of integrating rural crowd workers and providing  professional development in crowd markets. %3) new models for work and worker improvement that may generalize to other domains and problems. 





%be able to grow and develop themselves. 
\vf{I think you have something more general. That is, the proposed research will develop general techniques to enable paid-learning using crowd-markets.}
\vf{state here that you will create an alternative to online education using crowd markets explicitly. Also, how does this idea solves the problem you stated earlier?}.

\vf{Suggestion. For instance, people in rural communities believe that} Time spent learning online is time that the learner is not earning money. Therefore, online learning is not a feasible option for everyone, especially rural adults who cannot afford to not receive money to maintain their families. Online crowd markets have the potential of helping people learn new technical skills while working online. However, professional development on crowd markets is rare due to critical problems\vf{limitations?} in current platforms. \vf{What are the limitations/problems?} The open calls, short contracts, and lack of opportunities for workers to develop or distinguish themselves result in viscosity and stagnation that pushes effective wages low and keeps them there \vf{where is there?} without any opportunity for growth \vf{I don't understand the purpose of the past sentence. Not clear how it fits your proposal. It sounds more like a sentence that goas in the broader impact section.}. This proposal's research objective is to investigate interactive systems and computational techniques that transform crowd markets into platforms that enable professional growth while completing paid crowd work \vf{state here that you will create an alternative to online education using crowd markets explicitly. Also, how does this idea solves the problem you stated earlier?}. 

facilitate learning and professional growth on crowd markets. 




rural crowd workers are rare today due to critical problems \vf{I guess problems are ``technical challenges''?} in current crowd markets. The open calls, short contracts, and lack of opportunities for workers to develop or distinguish themselves result in viscosity and stagnation that pushes effective wages low and keeps them there.


The goal of this proposal is to investigate the development of workforce development in rural areas by leveraging crowd marketplace as an alternative to online learning

This proposal's research objective is to investigate interactive systems and computational techniques that 
facilitate learning and professional growth on crowd markets. 

integrate rural workers into crowd markets by facilitating professional development on these platforms \vf{The objective should be stated earlier.}

This proposal's research objective is to investigate interactive systems and computational techniques that integrate rural workers into crowd markets by facilitating professional development on these platforms \vf{The objective should be stated earlier.}

However, rural crowd workers are rare today due to critical problems \vf{I guess problems are ``technical challenges''?} in current crowd markets. The open calls, short contracts, and lack of opportunities for workers to develop or distinguish themselves result in viscosity and stagnation that pushes effective wages low and keeps them there. Consequently, rural workers who do join crowd markets, suffer from not receiving adequate salaries or learning how to make a living on these platforms. \vf{Are the two sentences before explaining the technical challenges? It is not clear.} 


everyone can afford to participate in online learning \vf{I think you mean: Thus, online learning is not a feasible option for a rural adult.}.

Frankola \cite{frankola2001online} claimed that adult learners drop out of online courses due to the lack of time, lack of management oversight, lack of motivation, problems with technology, lack of student support, individual learning preferences, poorly designed courses, and substandard or inexperienced instructors.


Online student retention has been suggested as one of the greatest weaknesses in online education

and to the decline of student achievement across the U.S. compared to other industrialized nations. Creating skilled workers for an economy that is constantly changing will require strategic investments and better education and workforce development programs, which must be coordinated and aligned with employers' needs.

Online education has enabled more people to have access to up-to-date curricula, empowering individuals to have better job opportunities, professional and academic growth. Online education has been especially transformative in rural regions. The majority of online education platforms consider settings where the learner has therefore to devote time for learning without earning money while they learn. This approach, however, is inadequate for people 

Yet, as online courses continue to be developed, many suggest a major challenge lies in the retention of students in these courses

Online student retention has been suggested as one of the greatest weaknesses in online education

Online student retention has been suggested as one of the greatest weaknesses in online education

Frankola \cite{frankola2001online} claimed that adult learners drop out of online courses due to the lack of time, lack of management oversight, lack of motivation, problems with technology, lack of student support, individual learning preferences, poorly designed courses, and substandard or inexperienced instructors.

%\textbf{However, time spend\vf{spent?} learning online is time that the rural adult is not earning money. As a result, not everyone can afford to participate in online learning \vf{I think you mean: Thus, online learning is not a feasible option for a rural adult.}}


**************************
\vf{Overall comments: \\ 1 . The motivation may be large, it takes quite a while to really read what you are proposing. I think you can shorten it by saying that online learning platforms have failed to prepare workforce development in rural areas because X, and Y. Then you say, we propose to use crowd markets as an alternative solution to get money while learning.\\ 2. Is there a theory or grounds that suggests that this approach will be successful? This should be discussed in the introduction though. If there is not, then at least mention a few studies showing that this direction can be promising. \\ 3. Given that is so focused on rural communities, I sense that some reviewers will say that this is not general. You may want to consider generalized this for any person, and then mention that you will be focusing on rural areas since this is a great tool for them and good for testing this approach.}

Adults from rural areas face challenges in the workplace. Most cannot find jobs in their communities and need to leave\vf{where? I guess you meant to say need to move to get opportunities elsewhere?}; or never receive training for the skills needed by the job market\vf{I would suggest finishing the sentence here, and say that as a consequence of these challenges they have limited employment opportunities in a new sentence}, and have limited employment choices. To date, the dominant approach to overcome these problems has been to provide online courses that give access to more relevant knowledge for the job market. However, time spend\vf{spent?} learning online is time that the rural adult is not earning money. As a result, not everyone can afford to participate in online learning \vf{I think you mean: Thus, online learning is not a feasible option for a rural adult.}. To extend the investigations on professional development, the proposed research studies the integration of rural adults as core members of crowd marketplaces \vf{1) I think it sounds clearer and more direct if you say the following: The goal of this proposal is to investigate the development of workforce development in rural areas by leveraging crowd marketplace as an alternative to online learning; 2) Could you briefly describe what a crowd marketplace is or some examples for clarity?}. Through this \vf{What is ``this''? Say directly what it means to avoid confusions}, rural adults might not need to abandon their communities and could learn new skills while getting paid to do crowd work. However, rural crowd workers are rare today due to critical problems \vf{I guess problems are ``technical challenges''?} in current crowd markets. The open calls, short contracts, and lack of opportunities for workers to develop or distinguish themselves result in viscosity and stagnation that pushes effective wages low and keeps them there. Consequently, rural workers who do join crowd markets, suffer from not receiving adequate salaries or learning how to make a living on these platforms. \vf{Are the two sentences before explaining the technical challenges? It is not clear.} This proposal's research objective is to investigate interactive systems and computational techniques that integrate rural workers into crowd markets by facilitating professional development on these platforms \vf{The objective should be stated earlier.}. Four objectives \vf{goals?} embody this approach. The first focuses on understanding how to integrate rural communities in crowd work. First, we will conduct in-lab and long-term studies to understand how rural adults could benefit from crowd markets, the problems they face in using current platforms, and how new tools may be beneficial. The next objectives will focus on enabling career development in crowd markets. Second, we will develop ``skill ladders'' that  enable skill development while doing crowd work. Third, we will create ``micro-mentoring'' tools that allow crowd workers to receive human mentoring from experts to further help their careers but without creating a burden on experts. Fourth, we will develop tools that help workers to present themselves to employers to have better job opportunities inside and outside crowd marketplaces. To accomplish these objectives, the PIs will follow a user-centered design process and execute longitudinal evaluations in the wild. Our studies will focus on benefiting adults in rural communities, a population that is in disadvantage in the current job market. We will also include adults from  other groups to increase the likelihood that our results will generalize. \vf{This sounds like you are minimizing the general public, and does not show much of an ambition from this proposal.}

{\bf Intellectual Merit:}
This research will introduce the first general techniques for: a) integrating rural workers into crowd markets; and b) facilitating workers' professional growth directly on existing crowd markets. This extends the boundaries of crowdsourcing research, which has focused on empowering requesters. Research that does look at workers has studied more the design of new crowd markets, or helping workers to organize. To accomplish these objectives, this research will produce: 1) techniques and patterns to facilitate the participation of rural workers and enable professional growth in crowd markets; 2) scientific results that uncover the strengths and weaknesses of integrating rural crowd workers and providing  professional development in crowd markets. %3) new models for work and worker improvement that may generalize to other domains and problems. 
This proposal is centered in crowdsourcing research, contributing to disciplines including HCI, social computing and computer-supported cooperative work.


{\bf Broader Impact:}
Most rural adults face difficulty succeeding in the current workforce. Our research may contribute to an additional type of employment opportunity for rural adults. Additionally, making crowd work better for workers is likely to impact a number of groups who either currently engage in crowd work or who may do so in the future, {\em e.g.}, stay-at-home parents, people with disabilities or older adults who could benefit from extra income. We will release the tools we develop as open source and deploy them so that people who could benefit from them can do so. \vf{Maybe include a few outreach activities?}





]*************************************************************
Over 70\% of United States' land area belongs to rural counties, and over 46.2 million Americans live in these areas. While there are programs to facilitate the education of children in rural communities, many 


%Crowd work seems to be an appropriate employment option for rural adults, especially, as they can continue to live in their communities.  Crowd work eliminates coming into an office every day, or needing to have in-person interactions. This proposal imagines a future where adults from rural communities can earn money without abandoning their towns, and while gradually learning new valuable skills, thus empowering rural workers to be relevant for the job market and have more  options. The broader context of this proposal is in the on-going changes to work. For many people, work is already becoming more flexible -- stay-at-home parents and other caregivers fit in time to work when they are able; some individuals in rural communities already in fact work remotely to avoid the difficulty of a commute. However, despite its potential advantages, current crowd platforms also have problems. The open calls, short contracts, and lack of opportunities for workers to develop or distinguish themselves result in viscosity and stagnation that pushes effective wages low and keeps them there. This proposal is about developing, deploying, and studying systems that will allow people to benefit from the advantages of crowd work while minimizing the current costs. We will especially target our work to benefit adults in rural communities, a population that is in disadvantage in the current job market. We will also include adults from cities and other groups to increase the likelihood that our results will generalize.

%We will : {\em (i)} conduct in-lab and long-term studies to understand how adults from rural communities could benefit from crowd working platforms, the problems they face in using current platforms, and how new tools may be beneficial; {\em (ii)} develop ``skill ladders'' to help workers improve their current skills and develop new skills while they work; {\em (iii)} create ``micro-apprentinship'' tools that allow workers to connect and receive mentoring from experts who further help the career development of workers; and {\em (iv)} develop tools that help workers to better present themselves to employers to have better employment opportunities inside and outside crowd marketplaces. 







this approach struggles in developing up-to-date curricula. Additionally, 


Adults from rural communities face challenges in the workplace. Most cannot find jobs in their communities and need to move. Many also never receive adequate training to have the skills needed for the job market,  and,  consequently, have less employment choices. Crowd work seems to be an appropriate employment option for rural adults, especially, as they can continue to live in their communities.  Crowd work eliminates coming into an office every day, or needing to have in-person interactions. This proposal imagines a future where adults from rural communities can earn money without abandoning their towns, and while gradually learning new valuable skills, thus empowering rural workers to be relevant for the job market and have more  options. The broader context of this proposal is in the on-going changes to work. For many people, work is already becoming more flexible -- stay-at-home parents and other caregivers fit in time to work when they are able; some individuals in rural communities already in fact work remotely to avoid the difficulty of a commute. However, despite its potential advantages, current crowd platforms also have problems. The open calls, short contracts, and lack of opportunities for workers to develop or distinguish themselves result in viscosity and stagnation that pushes effective wages low and keeps them there. This proposal is about developing, deploying, and studying systems that will allow people to benefit from the advantages of crowd work while minimizing the current costs. We will especially target our work to benefit adults in rural communities, a population that is in disadvantage in the current job market. We will also include adults from cities and other groups to increase the likelihood that our results will generalize.

We will : {\em (i)} conduct in-lab and long-term studies to understand how adults from rural communities could benefit from crowd working platforms, the problems they face in using current platforms, and how new tools may be beneficial; {\em (ii)} develop ``skill ladders'' to help workers improve their current skills and develop new skills while they work; {\em (iii)} create ``micro-apprentinship'' tools that allow workers to connect and receive mentoring from experts who further help the career development of workers; and {\em (iv)} develop tools that help workers to better present themselves to employers to have better employment opportunities inside and outside crowd marketplaces. 




{\bf Intellectual Merit:}
Research on rural adults has only begun to look at digital work, and has not considered improvements that would specifically help this population leverage crowd work, despite its promise and prevalence. Most work in crowdsourcing, especially tool development, has approached the problem from the point of view of requesters. Research that considers workers has focused on understanding workers, developing new platforms, or helping workers organize. Our work will consider how systems can be developed on top of existing platforms to allow workers to efficiently acquire new skills, learn from experts, and benefit from their expertise. Doing so will require developing new models for work and worker improvement that may generalize to other domains and problems.




{\bf Broader Impact:}
Over 70\% of United States' land area belongs to rural counties, and over 46.2 million Americans live in these areas. While there are programs to facilitate the education of children in rural communities, many rural adults face difficulty succeeding in current workforces. Our research may contribute to an additional type of employment opportunity for rural adults. Making crowd work better for workers is likely to be impactful for a number of groups who either currently engage in crowd work or who may do so in the future, {\em e.g.}, stay-at-home parents and other caregivers, or older adults who could benefit from extra income during retirement. We will release the tools that we develop as open source and deploy them so that people who could benefit from them can do so.


*****************************
to help workers improve their current skills and develop new skills while they work;



{\em (ii)} create a machine learning task recommendation engine and a user-facing queueing tool to help workers find suitable work efficiently and reduce the unpaid time workers spend ``finding" work rather than doing work; {\em (iii)} develop ``skill ladders'' to help workers improve their current skills and develop new skills while they work; and {\em (iv)} create tools that allow crowd workers with autism to work together to find work, share work, and exchange tips on working better together.




Adults in rural communities face challenges in the workplace.
In fact, some rural adults are already working on existing crowd work marketplaces.
This proposal imagines a future in which adults with autism are able to work from home as they are able, earning money to supplement and eventually replace disability supplements, while gradually learning new valuable skills.


In fact, some are already working on existing platforms. Crowd work eliminates the need to adhere to a fixed schedule, reduces or eliminates the need for in-person social interaction, and can be regularized so that new or unexpected situations  are reduced. This proposal imagines a future in which adults with autism are able to work from home as they are able, earning money to supplement and eventually replace disability supplements, while gradually learning new valuable skills.
%AG: the "seems" in third sentence doesn't sound convincing. Also, I don't think it's appropriate to frame ASD as disability in the last sentence.


%Crowd work generally offers a unique proposition for work. The ability to work from home when convenient, avoid the frustration of navigating inaccessible transportation

The broader context of this proposal is in the on-going changes to work. For many people, work is already becoming more flexible -- stay-at-home parents and other caregivers fit in time to work when they are able; some people with disabilities work remotely to avoid the difficulty of a commute; and some people with autism are able to work effectively on their own without navigating the social norms of a traditional workplace. Despite its potential advantages, current crowd platforms also have problems. The open calls, short contracts, and lack of opportunities for workers to develop or distinguish themselves result in viscosity and stagnation that pushes effective wages low and keeps them there.

This proposal is about developing, deploying, and studying systems that will allow people to benefit from the advantages of crowd work while minimizing the current costs. We will especially target our work to benefit adults with autism, a growing population that has already found some success with crowd work. We will also include adults without autism in order to increase the likelihood that our results will generalize.

